Discrete and Continuous Wigner Functions in Open Quantum Systems: Non-Markovian and Thermodynamic Effects

The central aim of the thesis is to examine how non-classical resources in finite-dimensional quantum systems can be identified, characterized, and protected for practical use in the presence of realistic noise. Using the discrete Wigner functions (DWFs) framework, we introduce negative quantum states and examine how their Wigner negativity, mana, coherence, and teleportation fidelity evolve under unital and non-unital channels, with particular attention to non-Markovian random-telegraph and amplitude-damping dynamics. We also analyze protection strategies based on weak measurement and quantum measurement reversal, showing that these methods can enhance quantum correlations, reduce fidelity deviation, and improve teleportation performance for two-qubit negative states in memory-bearing environments. Moreover, we demonstrate that certain negative states, derived from phase-space point operators, exhibit greater resilience than Bell states in measures of entanglement under non-Markovian noise. Further, this thesis focuses on developing and implementing quantum circuits for generating these states on superconducting hardware and realizing them for the first time on IBM's ibm-Brisbane device. Their preparation is verified using quantum state tomography, demonstrating high fidelity under realistic noise conditions. We propose a teleportation scheme that leverages one of the two-qubit negative quantum states as a resource. Moreover, these two-qubit negative quantum states are also found to perform better than the Bell states for maximal CHSH violation and Fisher information in noisy conditions. We believe that these negative quantum states have the potential to be used in place of the traditional Bell states in scenarios where non-Markovian errors are prevalent. (continued in the PDF)

==> preliminaryPages/acknowledgments.tex <==
\setmainfont[ Path = font/,
 BoldFont={CandaraBI}, 
 ItalicFont={booki},
 BoldItalicFont={bookbi}
 ]{bookr}
\addcontentsline{toc}{chapter}{Acknowledgements}

\begin{flushright}
\huge{\textbf{Acknowledgements}}
\end{flushright}


“When you want something, all the universe conspires in helping you to achieve it.” – Alchemist by Paulo Coelho.\\

I would like to begin by expressing my sincere gratitude to my senior secondary school teachers, Chatar Singh Sir and Renu Ma’am, who introduced me to the core science subjects in an engaging, intuitive, and enjoyable manner. Their teaching laid the foundation for my curiosity-driven approach to learning and ignited my desire to understand the fundamental workings of nature. With the unwavering support of my parents and what I believe to be the guiding hand of the Universe, I was able to pursue a career in science. I remain deeply thankful to Almighty God for blessing me with the strength, hope, and courage to embrace the opportunities that have shaped me at this stage of my life.\\

I am profoundly grateful to Prof. Subhashish Banerjee, my Ph.D. thesis supervisor, for accepting me as a member of his research group and for his constant mentorship throughout my doctoral journey. His deep research insight, invaluable guidance, and constructive feedback have played a pivotal role in shaping my scientific thinking and personal growth. He introduced me to the fascinating areas of discrete Wigner functions and open quantum systems, and entrusted me with the responsibility of extracting meaningful results from these frameworks. I sincerely thank the members of my SRC Committee, Assoc. Prof. Prabhat K. Jaiswal, Assoc. Prof. K. J. George and Assoc. Prof. V. Narayanan, for their thoughtful suggestions, critical evaluations, and continued encouragement during various stages of my research.\\

Collaborations play a crucial role in broadening perspectives and fostering multidisciplinary learning in research. I feel extremely fortunate to have collaborated with Dr. K. G. Paulson and Dr. Pavitharan Iyer during my Ph.D. work. I distinctly recall a challenging phase during my third year, when I felt directionless and struggled to obtain new results. Dr. Paulson’s reassuring words, “Jayaa, I think you have done enough good work, and I know you will be getting many more amazing results. I have faith in you,” helped dispel my self-doubt and motivated me to work with renewed determination. From him, I learned the importance of logical thinking, productivity, and, most importantly, self-belief, the conviction that I can make meaningful contributions to the research community in my own way. These lessons proved instrumental in my research journey.\\

Labmates significantly influence the quality of one’s Ph.D. experience, and I feel privileged to have shared this journey with wonderful colleagues. I would like to acknowledge my close friends Devvrat and Baibhab for their constant support, kindness, and companionship, which made the demanding phases of my Ph.D. more manageable. I extend special thanks to Devvrat for being a patient and peaceful listener. His belief that “have faith in yourself and work hard so that you can do something for humanity” continually inspired me to strive for self-improvement. He also helped me understand several technical aspects of my research. I fondly cherish the scientific as well as spiritual discussions shared over tea with Devvrat and Baibhab.\\

I am also thankful to my seniors Ramniwas, Muskan, and Monika, and my junior colleagues and friends Mahima, Nihar, and Soyam, for creating a friendly, supportive, and intellectually nourishing lab environment. Special thanks to Mahima and Nihar for taking care of me like family during times of illness.\\

Over the past five years, I have built many meaningful connections within the Department of Physics, IIT Jodhpur. I would like to express my heartfelt thanks to my dear friends Sushma, Shikha, Hema, Abhijit, Abhishek, Ritesh, Anil, Debasish, Shubham, Surbhi, Priyambda, Jitendra, Sapta, Bikram, and Chayan, who made my time at IIT Jodhpur both enjoyable and memorable. I also deeply cherish the countless moments of laughter and warmth shared with Bhawna Di, Mahima, and Lekha, which added joy to my life on campus.\\

I gratefully acknowledge the unwavering support of my graduation friends Preeti, Minakshi, and Sangeeta, who have been an integral part of not only my academic journey but also my emotional well-being. Their presence transcended friendship; they stood by me like family during every phase of this journey.\\

I humbly dedicate this Ph.D. to my Mummy and Papa, whose love, sacrifices, and unconditional support made this achievement possible. Although quantum physics was beyond the scope of our daily conversations, their constant concern for my well-being, ensuring that I was healthy, safe, and well-fed, gave me the emotional stability to persevere. This doctoral journey would not have been possible without their faith in me.\\

Finally, I would like to acknowledge my brothers Vikas, Vinod, and Shubu, my sister-in-law Jyoti, and Sinu for taking such good care of me throughout my Ph.D. years. I also thank my sisters Khushu, Indu, and Poonam for being steadfast pillars of support during challenging times. I am deeply grateful to my Tau ji and Mosi ji for their constant encouragement and belief in me, which served as a continuous source of strength.\\

Thank you, Universe.

\begin{flushright}
\authorname  \\
Ph.D. Student
 
\end{flushright}



 
 
 





==> preliminaryPages/certificate.tex <==
\setmainfont[ Path = font/,
 BoldFont={CandaraBI}, 
 ItalicFont={booki},
 BoldItalicFont={bookbi}
 ]{bookr}


 


\begin{flushright}
\huge{\textbf{Certificate}}
\end{flushright}
  This is to certify that the thesis titled "\emph{\ttitle{}}", submitted by \authorname{} (\rn{}) to the Indian Institute of Technology Jodhpur for the award of the degree of \degree{}, is a bonafide record of the research work done by her under my supervision. To the best of my knowledge, the contents of this report, in full or in parts, have not been submitted to any other Institute or University for the award of any degree or diploma.
\vspace{2cm}
\begin{flushright}
\large{\textbf{Signature}}\\
\supname\\
Ph.D Thesis Supervisor 
\end{flushright}

==> preliminaryPages/declaration.tex <==
\setmainfont[ Path = font/,
 BoldFont={CandaraBI}, 
 ItalicFont={booki},
 BoldItalicFont={bookbi}
 ]{bookr}


 

% ItalicFont

\begin{flushright}
\huge{ \textbf{Declaration}}
\end{flushright}
{ I hereby declare that the work presented in this thesis titled ``\emph{\ttitle{}}", submitted to the Indian Institute of Technology Jodhpur in partial fulfilment of the requirements for the award of the degree of~ \degree, is a bonafide record of the research work carried out under the supervision of \supname. The contents of this thesis, in full or in parts, have not been submitted to, and will not be submitted by me to, any other Institute or University in India or abroad for the award of any degree or diploma.}
\vspace{2cm}
\begin{flushright}
\large{\textbf{Signature}}\\
\emph{\authorname}\\
\rn
\end{flushright}


==> preliminaryPages/nomenclature.tex <==
%\newpage

\renewcommand{\nomname}{List of Symbols}
\addcontentsline{toc}{chapter}{List of Symbols}
\setlength{\columnsep}{4pc}
\setstretch{0.5}

% Refer to https://www.overleaf.com/learn/latex/Nomenclatures#Sorting_the_Entries for more info

% Define nomenclature entries with grouping
\renewcommand\nomgroup[1]{%
  \item[\bfseries
  \ifstrequal{#1}{P}{Physics constants}{%
  \ifstrequal{#1}{N}{Number sets}{%
  \ifstrequal{#1}{O}{Other symbols}{}}}%
]}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{multicols}{2}
%%% Include the nomenclature section
\nomenclature[O]{\rho}{Density \nomunit{(Kg/$m^3$)}}  % without numbering
\nomenclature[P, 01]{v}{Speed of sound \nomunit{(m/s)}} % with unit
\nomenclature[P, 01]{c}{Speed of light in a vacuum} % with numbering
\nomenclature[P, 02]{$\hbar$}{Planck constant}
\nomenclature[P, 03]{G}{Gravitational constant}
\nomenclature[P, 04]{RH}{relative humidity in percentage}
\nomenclature[N, 05]{\mathbb{R}}{Real numbers}
\nomenclature[N, 06]{\mathbb{C}}{Complex numbers}
\nomenclature[N, 07]{\mathbb{H}}{Quaternions}
\nomenclature[O, 08]{V}{Constant volume}
\nomenclature[O, 09]{\nu}{Friction index}

\end{multicols}





%\printglossary[type=\acronymtype]
%\printglossary[title={List of Abbreviations}] %Generate List of Abbreviations
%\renewcommand{\nomname}{List of Symbols}
%\renewcommand{\nomname}{Nomenclature}
%\begin{singlespace}
%\printnomenclature
%\end{singlespace}


% Add the Print the nomenclature at the end 
\printnomenclature
